KARL: Kalman-Filter Assisted Reinforcement Learner for Dynamic Object Tracking and Grasping

We present Kalman-filter Assisted Reinforcement Learner (KARL) for dynamic object tracking and grasping over eye-on-hand (EoH) systems, significantly expanding such systems capabilities in challenging, realistic environments. In comparison to the previous state-of-the-art, KARL (1) incorporates a novel six-stage RL curriculum that doubles the system's motion range, thereby greatly enhancing the system's grasping performance, (2) integrates a robust Kalman filter layer between the perception and reinforcement learning (RL) control modules, enabling the system to maintain an uncertain but continuous 6D pose estimate even when the target object temporarily exits the camera's field-of-view or undergoes rapid, unpredictable motion, and (3) introduces mechanisms to allow retries to gracefully recover from unavoidable policy execution failures. Extensive evaluations conducted in both simulation and real-world experiments qualitatively and quantitatively corroborate KARL's advantage over earlier systems, achieving higher grasp success rates and faster robot execution speed. Source code and supplementary materials for KARL will be made available at: https://github.com/arc-l/karl.

==> texs/02-backup.tex <==
\subsection{Overview of EARL\cite{earl}}
The EARL framework was designed to address the challenges of dynamic object grasping using an Eye-on-Hand (EoH) system. It features a fully integrated perception and manipulation system, eliminating workspace constraints and occlusion issues that are typical of external camera setups. Given that a stable grasp can become unreachable as the object moves, EARL integrated real-time object tracking, grasp planning, and reinforcement learning (RL) to dynamically adapt to object motion without requiring explicit motion prediction. 
% EARL was developed to tackle the challenges of dynamic object grasping using an Eye-on-Hand (EoH) system. It integrates perception and manipulation, eliminating workspace constraints and occlusion issues typical of external camera setups. Since a stable grasp may become unreachable as the object moves, EARL employs real-time object tracking, grasp planning, and reinforcement learning (RL) to continuously adapt without requiring explicit motion prediction.

\subsection{Real-Time Object Tracking and Pose Estimation}
An RGB-D sensor mounted on the robotic arm enables EARL to track objects in real-time. It leverages R2D2~\cite{r2d2}, enhanced with BundleTrack~\cite{bundletrack}, which maintains keyframe memory and optimizes 6D pose estimation in real-time.
% Equipped with an RGB-D sensor mounted on the robotic arm, EARL employs a correspondence-based tracking method named R2D2~\cite{r2d2}, enhanced with BundleTrack~\cite{bundletrack}, to maintain a keyframe memory and optimize 6D pose estimation in real-time.  
\subsection{Grasp Planning and Adaptation}
EARL ensures adaptable grasping through Contact-GraspNet~\cite{contact_grasp_net}, which generates multiple 6-DoF grasp candidates without requiring prior object models. These candidates are stored in a grasp memory pool, allowing the system to select the most stable and reachable grasp based on real-time object pose changes.
% To ensure adaptable grasping, EARL utilizes Contact-GraspNet~\cite{contact_grasp_net}, which proposes multiple 6-DoF grasp candidates without relying on prior object models. These candidates are stored in a grasp memory pool, allowing the system to dynamically select the most stable and reachable grasp based on real-time pose changes. 
\subsection{Real Robot System and Target Object Workspace}
The real robot system consists of a UR5e robotic arm (6-DOF) controlled by directly specifying joint velocities, with an Intel RealSense L515 RGB-D camera mounted near the end-effector for real-time perception.  Grasping is performed using a Robotiq 2F-85 two-finger gripper, and the target object's workspace is defined as a 40 × 40 × 40 cm³ cubic region along the X, Y, and Z axes respectively.
% For grasping, EARL uses a Robotiq 2F-85 two-finger gripper. The workspace for the target object was defined as a cubic region with dimensions 40 × 40 × 40 cm³ along X, Y, Z axes respectively.
\subsection{Reinforcement Learning and Control Policy}
The 6D pose feedback from the perception system, along with the robot’s joint states, enables a Proximal Policy Optimization (PPO)-based policy to generate joint velocity commands and gripper actions~\cite{ppo}. EARL employs a curriculum-driven RL approach to ensure efficient tracking, collision avoidance, and precise grasp execution. To achieve robust grasping, reward shaping is carefully designed with multiple objectives:

% The 6D pose feedback from the perception system coupled with the robot's joint states enables a Proximal Policy Optimization (PPO~\cite{ppo})-based control policy to generate joint velocity commands and appropriate gripper actions. EARL's curriculum trained RL strategy is designed to balance efficient tracking, collision avoidance, and precise grasp execution. To ensure effective reward shaping, EARL's reward function incorporates multiple components that guide the robot’s behavior:
\begin{itemize}
    \item \textbf{Tracking and View Maintenance:} A penalty is assigned when the target object moves out of view, reinforcing active object tracking. 
    \item \textbf{Collision Avoidance:} A penalty to discourage pre-grasp collisions while ensuring the gripper remains within an effective range.
    \item \textbf{Grasp Execution:} Rewards the agent for closing the gripper at the optimal moment based on contact force detection.
    % The system dynamically determines the optimal moment to close the gripper, with a reward assigned upon successful grasp detection.
    \item \textbf{Alignment and Approach:}  Encourages proper gripper alignment along multiple axes (Y \& Z) to maximize grasp stability.
    % Regularization terms encourage proper gripper alignment along multiple axes to facilitate robust grasping.
\end{itemize}

\subsection{Training and Simulation Environment}
EARL utilizes parallel training of a single PPO agent on the rigid body simulation platform Isaac Gym~\cite{isaacgym}, allowing RL training at 65000+ mean FPS with 8192 parallel environments on a single RTX 4090 GPU. The action space is discrete and the robot's policy is a 3-layer MLP. The simulated objects were sourced from the YCB~\cite{ycb} and HOPE~\cite{hope} datasets. In the real-world execution, EARL can generalize to other objects as the perception system deployed does not require CAD models to perform object tracking.
\subsection{Evaluation}
EARL was evaluated in both simulation and real-world experiments. The object’s pose was directly provided by the simulator, with each trial consisting of a single grasp attempt. In real-world testing, objects moved in predefined trajectories—linear, oval, or random—with an additional static object scenario. The task was deemed successful if the robot grasped and lifted the moving object. The object’s translation speed was capped at 6 cm/s, and the grasp success rate was defined as the percentage of successful grasps within a specified time limit (35 seconds). Failures were categorized as collisions, loss of object tracking, or exceeding the maximum episode duration (35 seconds).


\subsection{Limitations of the EARL Curriculum and Overall System}

While the three-stage curriculum progressively increases task difficulty, overall grasping success can be improved across various object motion profiles, including fixed (e.g., linear) and random patterns, as well as scenarios involving higher object speeds. The initial stage overly imposes restrictive starting positions for the robot, limiting its exposure to diverse object configurations and slowing adaptation. In later stages, strong penalties for objects moving out of view and for collisions discourage necessary exploration, making the robot overly conservative and highlighting opportunities to improve both grasping speed and accuracy. Additionally, weak alignment penalties lead to less stable hand-object positioning. Although EARL demonstrated real-time dynamic grasping, it exhibits several limitations:
\begin{itemize}
    \item Slower, unrealistic \textbf{robot speeds}, limiting rapid adaptation in dynamic environments.
    \item Slower than usual \textbf{object speeds} (2–6 cm/s), which do not fully reflect real-world object handovers, where humans tend to move objects at slightly higher speeds.
    \item A 35-second grasping \textbf{time limit}, which is longer than practical requirements—a 20-second limit would be more realistic.
    \item Inability to \textbf{recover objects} once they move out of the camera’s field of view, restricting grasping performance in complex scenarios with unpredictable object motion.

\end{itemize}

In KARL, the integration of perception, manipulation, and policy simulation modules remains largely unchanged, as we continue using the EoH system. However, enhancements within these modules address the limitations identified in EARL.


% \subsection{Limitations of EARL Curriculum and Overall system}
% While the three-stage curriculum guided training by progressively increasing task difficulty, overall grasping success can be improved across different object motion profiles (fixed patterns like line or random patterns) and for object motions involving higher speeds. The initial stage overly restricted the robot’s starting position, limiting exposure to diverse object configurations and slowing adaptation. In later stages, strong penalties for the object going out of view and collisions discouraged necessary exploration, making the robot overly conservative and demonstrating a room for improving both grasping speed and accuracy. Additionally, weak alignment penalties display less stable hand-object positioning. While EARL demonstrated real-time dynamic grasping, it exhibited limitations such as:


% \begin{itemize}
%     \item Slower, non-realistic \textbf{robot speeds}, limiting rapid adaptation to dynamic environments.
%     \item Lower-than-average \textbf{object speeds} (2–6 cm/s), which do not fully capture real-world object motion challenges.
%     \item A 35-second grasping \textbf{time limit}, which is slower than practical requirements—a 20-second limit would be more realistic.
%     \item Inability to {recover objects} once they leave the camera’s field of view, restricting grasping in complex scenarios where objects move unpredictably.
% \end{itemize}
% In KARL, the integration of the perception, manipulation and policy simulation modules within the pipeline remains largely unchanged, as we retain the use of the EoH system. However, enhancements have been made within these modules to overcome the limitations identified in EARL.



% The performance of EARL was evaluated through both simulation and real-world robotic experiments. In the simulated environment, the object's pose was provided by the simulator, and each trial consisted of a single grasp attempt. The experimental setup involved objects moving in predefined linear, oval, or random trajectories, with an additional static object scenario.
% Experiments also involved an additional scenario where the object remains static. 
% The task was considered successful if the robot successfully grasped and lifted the moving object. Object's translation speed was capped at 6 cm/s. EARL's effectiveness was measured by the grasp success rate, defined as the percentage of successful grasps within a specified time limit. Three failure conditions were recorded: collision, loss of target object tracking, and reaching the maximum episode duration (35 seconds).
% demanding  more realistic conditions, 

% \begin{itemize}
%     \item \textbf{Higher robot speeds}, requiring quicker and more stable grasp executions.
%     \item \textbf{Reduced grasping task time limits}, demanding rapid decision-making.
%     \item \textbf{Faster object velocities}, making tracking and grasping more challenging.
%     \item \textbf{Tracking Failures}, where the target frequently moves out of view of the EoH camera.
% \end{itemize}

    % Despite its effectiveness, EARL faces several limitations under more demanding conditions:
% KARL builds upon the EARL framework by refining reward shaping, perception, and control strategies to achieve superior grasping performance under these conditions. These enhancements enable more robust grasping in highly dynamic scenarios, ensuring that the system remains effective even when object motion is more erratic and time constraints are stricter.




% Because the object's velocity, as well as its initial and final positions, were predetermined, active pose estimation was unnecessary—the entire motion trajectory was known from the outset. However, to maintain a realistic simulation, the robot’s policy was designed without access to the full trajectory. Instead, it relied solely on the difference in the object's pose between consecutive time frames and the robot’s current joint states to generate appropriate movements.


% \subsection{Evaluation}
% EARL's performance was assessed in both simulation and real robot experiments. In simulation, the simulator provides the object's pose, and a single grasp attempt is made per trial. Since, the object's velocity, start and end poses are chosen in advance, an active pose estimation is not necessary as the object's motion trajectory is available from the beginning. However, the robot's policy (to simulate reality) is unaware of the full trajectory and only knows the pose difference between the current and previous time frame alongside the robot's current joint states in order to produce appropriate motion.   

% Experiment typically involves freely moving an object in fixed patterns like linear or oval or purely random motion, and in the end the task is considered successful when the robot accurately grasps and lifts the moving object. Object's translation speeds during experiments were limited to 6 cm/s. The success of the method is evaluated based on the grasp success rate, where the robot successfully grasps the target object within a predefined time limit (timeout). Three failure conditions are recorded:
% \begin{itemize}
%     \item Collision
%     \item Loss of target object tracking
%     \item Reaching the maximum episode length
% \end{itemize}

% Since active pose estimation is not employed in these simulation experiments, object visibility is determined by checking if the object's pose center moves beyond a threshold (~20°) from the camera's principal axis. Each trial has a maximum time limit of 35 seconds (timeout).  



% With the RGB-D sensor mounted on the robotic arm, EARL leveraged a correspondence-based tracking method, enhanced with BundleTrack, to maintain keyframe memory and optimize the target's pose estimation in real-time, allowing the control policy—trained via Proximal Policy Optimization (PPO)—to generate smooth and responsive joint velocity commands based on the object pose differentials. The system dynamically updates grasp proposals via Contact-GraspNet, which generates multiple grasp candidates without needing prior object models. These candidates are stored in a grasp memory pool, allowing the robot to adapt its grasp strategy based on angular distance and pose changes this ensures selecting the most stable and reachable candidate as the object moves in 6D space. 

% However, the EoH setup presents a unique challenge: since tracking relies on the arm-mounted camera, losing sight of the object results in tracking failure and, consequently, grasping failure. To mitigate this, we introduce a re-engagement mechanism that estimates the uncertainty of the object's pose using an Extended Kalman Filter~\cite{ekf}. This allows the robot to follow a predicted motion trajectory, eventually regaining sight of the object and reestablishing successful grasping. 
% In KARL, the perception, manipulation and policy's simulation training modules of the overall pipeline largely remain unaffected as the new setup is still an EoH system and improvements were made inside the respective modules to address the limitations of EARL.  

% KARL retains the core EoH setup and builds upon it, with the MLP network of the policy, core object tracking and grasping principles unchanged.


==> texs/03-backup.tex <==
\ours has three main, interconnected modules (see Fig.~\ref{fig:karl} for an illustration). The perception sub-system of \ours contains two of these components: an initial pose registration module and a continuous pose tracking/recovery module. The third module is the RL-based robot controller. 

\subsection{Initial Pose Registration}
\ours takes in request in the form of simple natural language inputs, e.g., ``robot, grab that \emph{milk carton}.'' Upon receiving a request, \ours prompts Grounding DINO~\cite{gdino} to automatically extract the target object from images taken from the EEF-mounted RGB-D camera. At this point ($t = 0$), two additional tasks are performed: initial pose estimation/registration and candidate grasp generation. For the former, FoundationPose~\cite{foundationpose} is invoked to perform the pose estimation of the target object using RGB-D and the object mask. Since FoundationPose is designed for offline/video-based pose estimation and tracking, we modify it for an online setting, enabling real-time 6D pose estimation with actively streamed image data. For the latter, Contact-GraspNet~\cite{sundermeyer2021contact} is applied directly to the (segmented) depth data to produce (a few) candidate grasps. Formally, given RGB-D and mask inputs $(\mathcal{I}_0, \mathcal{D}_0, \mathcal{M}_0)$, the initial pose registration phase yields Object's 6D pose $\mathcal{T}_0^{\mathcal{C}}$, and grasp pose candidates $\mathcal{O}_\text{pool}^{\mathcal{W}}$ in the Camera $\mathcal{C}$ and World Frames $\mathcal{W}$ respectively.

\textcolor{red}{Done - Add proper variable names for the object pose and grasp pose candidates}

\subsection{Real-Time Pose Tracking and Tracking Loss Recovery}
\subsubsection{Continuous Pose Tracking Before Tracking Loss} 
% For continuous pose tracking, we explored two approaches. One of these was adapt the pose tracking method from~\cite{earl}, which
Obtaining the initial pose estimate from FoundationPose~\cite{foundationpose}, we leverage a combination of R2D2~\cite{r2d2} and BundleTrack~\cite{bundletrack} from~\cite{earl} to track the object in real-time. 
% to sift through up to 60 pose hypotheses, sampled around the previous pose estimate. This method provides decent performance. 
%
For our second attempt, because FoundationPose~\cite{foundationpose} was shown to provide excellent pose estimation/registration results, it would be ideal if it can also be used for the continuous pose tracking task.  However, in the EoH setup where both the camera and target object move randomly in 3D space, the tracker in FoundationPose often becomes unstable. We attribute this to FoundaionPose's pose refiner model encountering object trajectories (from our setup) that were likely absent from its training data. 
%

\subsubsection{Tracking Loss Detection and Recovery} \textcolor{red}{todo}

\subsection{RL-Based Robot Controller}
\subsubsection{Reward Shaping and Curriculum Design} \textcolor{red}{todo}

\subsubsection{Grasp Failure Detection and Recovery} \textcolor{red}{todo}

\subsection{Improvements to the EARL Baseline} 
\textcolor{red}{todo - anything to be written here?}

\textcolor{red}{JJ's edit location}

% \subsection{Input Data}
% At each time step $t$, the system receives:
% \begin{align}
%     \text{rgb}_t &\in \mathbb{R}^{H \times W \times 3}, \quad \text{(RGB image from the camera)} \\
%     \text{depth}_t &\in \mathbb{R}^{H \times W}, \quad \text{(Depth map from the camera)} \\
%     \text{text\_prompt} &\in \mathcal{S}, \quad \text{(Semantic label of the target object)}
% \end{align}
% where $\mathcal{S}$ is a predefined set of possible object descriptions.

% \subsection{State Representation}
% The \textit{state vector} $\mathbf{x}_t$ of the object at time $t$ is represented as:
% \begin{equation}
%     \mathbf{x}_t = \begin{bmatrix} \mathbf{p}_t & \dot{\mathbf{p}}_t & \mathbf{q}_t & \boldsymbol{\omega}_t \end{bmatrix}^\top
% \end{equation}
% where:
% \begin{itemize}
%     \item $\mathbf{p}_t = [x, y, z]^\top$ is the object position.
%     \item $\dot{\mathbf{p}}_t = [v_x, v_y, v_z]^\top$ is the linear velocity.
%     \item $\mathbf{q}_t = [q_x, q_y, q_z, q_w]^\top$ is the orientation as a quaternion.
%     \item $\boldsymbol{\omega}_t = [\omega_x, \omega_y, \omega_z]^\top$ is the angular velocity.
% \end{itemize}
% The \textit{covariance matrix} $\mathbf{P}_t$ represents the uncertainty in the state estimate.

% \subsection*{Pose Estimation Pipeline}
% 1. **Object Detection and Pose Initialization:**
%    \begin{align}
%        B_0 &= \operatorname{GroundingDINO}(\text{rgb}_0, \text{depth}_0, \text{text\_prompt}) \\
%        M_0 &= \operatorname{2D\_Tracker\_Initialize}(\text{rgb}_0, B_0) \\
%        \mathbf{T}_0 &= \operatorname{FoundationPose\_Register}(\text{rgb}_0, \text{depth}_0, M_0)
%    \end{align}

% 2. **Tracking and Kalman Filtering:**
%    - If the object is in view:
%      \begin{align}
%          \mathbf{T}_t &= \operatorname{BundleTrack+R2D2}(\text{rgb}_t, \text{depth}_t, M_t, \mathbf{T}_{t-1}) \\
%          \mathbf{x}_t, \mathbf{P}_t &= \operatorname{EKF.update}(\mathbf{T}_t)
%      \end{align}
%    - If the object is not in view:
%      \begin{align}
%          \mathbf{T}_{\text{pred}, t} &= \operatorname{EKF.predict}() \\
%          \text{robot.move\_towards}(\mathbf{T}_{\text{pred}, t})
%      \end{align}
%    - If the object is reacquired:
%      \begin{align}
%          \mathbf{T}_{\text{recover}, t} &= \operatorname{FoundationPose}(\text{rgb}_t, \text{depth}_t, \mathbf{T}_{\text{pred}, t}) \\
%          \mathbf{x}_t, \mathbf{P}_t &= \operatorname{EKF.update}(\mathbf{T}_{\text{recover}, t})
%      \end{align}

% \subsection*{Extended Kalman Filter (EKF)}
% We use an **Extended Kalman Filter** to fuse pose estimates over time.

% **Prediction Step:**
% \begin{align}
%     \mathbf{x}_t &= \mathbf{F} \mathbf{x}_{t-1} + \mathbf{w}_t, \quad \mathbf{w}_t \sim \mathcal{N} (0, \mathbf{Q}) \\
%     \mathbf{P}_t &= \mathbf{F} \mathbf{P}_{t-1} \mathbf{F}^\top + \mathbf{Q}
% \end{align}

% **Measurement Update:**
% \begin{align}
%     \mathbf{y}_t &= \mathbf{z}_t - \mathbf{H} \mathbf{x}_t \\
%     \mathbf{S}_t &= \mathbf{H} \mathbf{P}_t \mathbf{H}^\top + \mathbf{R} \\
%     \mathbf{K}_t &= \mathbf{P}_t \mathbf{H}^\top \mathbf{S}_t^{-1} \\
%     \mathbf{x}_t &= \mathbf{x}_t + \mathbf{K}_t \mathbf{y}_t \\
%     \mathbf{P}_t &= (\mathbf{I} - \mathbf{K}_t \mathbf{H}) \mathbf{P}_t
% \end{align}

% \subsection*{Objective Function}
% The optimal state estimate $\mathbf{x}_t^*$ is obtained by minimizing the \textit{state estimation error}:
% \begin{equation}
%     \mathbf{x}_t^* = \arg \min_{\mathbf{x}_t} \sum_{k=0}^{t} \left\| \mathbf{z}_k - \mathbf{H} \mathbf{x}_k \right\|_{\mathbf{R}}^2 + \left\| \mathbf{x}_k - \mathbf{F} \mathbf{x}_{k-1} \right\|_{\mathbf{Q}}^2
% \end{equation}
% where $\|\mathbf{e}\|_{\mathbf{R}}^2 = \mathbf{e}^\top \mathbf{R}^{-1} \mathbf{e}$ is the Mahalanobis distance.

% EoH setup presents a unique challenge: since tracking relies on the arm-mounted camera, losing sight of the object results in tracking failure and, consequently, grasping failure. 
% To mitigate this, we introduce a re-engagement mechanism that estimates the uncertainty of the object's pose using an Extended Kalman Filter~\cite{ekf}. This allows the robot to follow a predicted motion trajectory, eventually regaining sight of the object and reestablishing successful grasping. 
% The proposed system is designed to improve the grasping success rate under faster robot speeds, larger target object workspaces, higher target object speeds with a failure recovery mechanism to recover successful grasping, when the object momentarily exits the camera view before the initial human to robot object handover is completed. 
\subsection{Objective}
The proposed system is designed to enhance grasping success rates by supporting faster robot speeds, larger target object workspaces, and higher object velocities. It also includes a failure recovery mechanism to re-establish a successful grasp if the object momentarily exits the camera's view before the human-to-robot object handover is completed.
% With this, the robot can continue to reach the target object even if it goes out of view. 
% A key advancement in KARL is out-of-view failure recovery. 
% , our system predicts the object's current pose to maintain continuity. The robot follows this pose until the object reappears, at which point it re-estimates the object's 6D pose and resumes the grasping attempt. This ensures a robust and adaptive approach to dynamic grasping, reducing failures due to temporary occlusions or rapid object movement. Finally, the task is considered successful when the robot accurately grasps and lifts the moving object. 

\subsection{Enhanced Grasping Policy}
\subsubsection{RL Curriculum and Reward Design}
\textcolor{red}{The terms for the rewards for each stage should be summarily, but clearly listed.}
% KARL utilizes parallel training of a single PPO agent on the rigid body simulation platform Isaac Gym~\cite{isaacgym}, allowing efficient RL training at 65000+ mean FPS with 8192 parallel environments on a single RTX 4090 GPU. The action space is discrete and the robot's policy is a 3-layer MLP.




We propose here a new reward shaping and curriculum design by identifying factors that positively influence the policy training outcomes. First off, a high reward of $180.0$ is given for successful grasping ($R_{grasp}$). A negative penalty that aims to decrease the distance between the robot and the target ($R_{dist}$) is set to $-1.0$. 
% When this encourages the robot to reach the target, a distance , while incorrect gripper alignment incurs a stronger penalty of $-6.0$ ($R_{keypoint_over}$). 
Misalignment of the gripper with the grasp pose of the object is discouraged with a penalty of $-0.015$ ($R_{align}$), and unnecessary actions are penalized at $-0.005$ ($R_{action}$). Collisions result in a penalty of $-1.5$ ($R_{collision}$), and failure to maintain object visibility incurs a penalty of $-1.5$ ($R_{view}$). Premature or incorrect gripper closure is penalized at $-0.3$ ($R_{gripper\_penalty}$). While the objective to keep object in view discourages the robot to staying too close to the object during excessive target object movement. To achieve grasping, staying too far from the target is also not desirable and hence a distance farther than 25 cms is discouraged with a penalty of $-0.25$ ($R_{dist\_over}$).

In stage zero, the robot starts in the center of the target workspace with target objects sampled closer to the robot. The primary focus is on trying to keep object in view and discouraging collisions before refining grasping skills and the robot is not stopped even if object goes out of view.  
In stage 1, strict object in view mode is activated when a sufficiently high reward threshold is reached, leading to an increase in penalty factors such as keypoint over-penalty (scaled by 6x), keep-object-in-view penalty (scaled by 10x), and collision penalty (scaled by 10x), while keypoint rewards and alignment penalties are doubled. The robot still starts in the center of the target workspace.

As training progresses, the curriculum encourages the system to handle more dynamic environments. Once the initial visibility constraints are met, the object's movement speed increases, first allowing up to 5 cm/s, then escalating to 12.5 cm/s in subsequent sub-phases in stage 2. The robot's starting position is gradually adjusted, moving from its initial placement to farther positions, ensuring it can handle larger workspaces. In parallel, key penalties and rewards continue to be scaled to reinforce effective grasping while discouraging unnecessary movements.

Further into training, a balance between speed and safety is introduced. When a higher reward threshold is met, safer movement constraints are imposed, increasing penalties on object tracking loss (6x further) and misalignment (2x further) while further refining grasp precision. The curriculum then progresses to a real adaptation stage where the object moves freely in all directions, requiring the robot to grasp dynamically with minimal restrictions. At this stage, the system transitions to keeping robot more responsive/faster. Once the policy achieves a high grasp success rate, fine-tuning phases begin. 

Fine-tuning phases ensure optimal grasp distance, gradually adjusting the target object movement distance penalty. If performance continues to improve, the environment is further stabilized by increasing penalties on object tracking loss (8x) and collisions(8x) while reinforcing proper alignment(2x more penalty). This final stage guarantees a robust grasping policy capable of handling high-speed object movements with a balance of precision, stability, and efficiency.
In summary, for early stages (0-1), high penalties are enforced for losing object visibility and collisions, moderate rewards for grasping. Mid-stages focus on Balancing speed and safety, with increasing importance of precision grasping. Late stages (5-6): Ensuring robustness by enforcing strict tracking and alignment penalties while maintaining high grasp success rates.

KARL introduces a six-stage curriculum with smoother performance-adaptive transitions between stages of the curriculum and improved reward shaping.  
The new curriculum enforces object visibility more aggressively in the initial phase, ensuring the robot learns to maintain sight of the object even before grasping skills are refined.
Instead of gradually increasing object speeds in training, we accelerate the object movements earlier in KARL, to promote faster adaptation to higher curriculum levels with faster object movements. The system also increases rewards for firm grasps upon correct alignment. Alignment and action penalties have been fine-tuned to discourage unnecessary movements, improving efficiency and reducing grasp failures due to misalignment. A late-stage fine-tuning phase reduces excessive penalties while reinforcing high-precision grasping, ensuring that fast object movements are not over-penalized. KARL ultimately strikes a better balance between speed, accuracy, and stability, enabling more effective grasping in high-speed conditions.
\subsubsection{Enlarged Target Object Workspace}

\subsection{Object Tracking with FoundationPose~\cite{foundationpose}}

%\textbf{Preliminaries}
\subsubsection{Problem Statement}
The robot receives at each time-step $t$ an RGB image $I_t$ and a depth image $D_t$ of a scene.
Given an object $O$ in the scene, our goal is to continuously estimate its \textit{6D pose} $\mathbf{T}_t$ over time using a combination of:
%\begin{enumerate}
    (1) visual object detection and tracking methods (Grounding DINO~\cite{gdino}, 2D tracker~\cite{2dTracker}, BundleTrack~\cite{bundletrack}+R2D2~\cite{r2d2}),
    (2) FoundationPose~\cite{foundationpose} for pose registration,
    and (3) Recursive state estimation with an \textit{Extended Kalman Filter (EKF)}~\cite{ekf} when the object is out-of-view.
%\end{enumerate}
The estimated pose is used to guide a robot towards the object for grasping.

\subsubsection{6D Pose Representation}
\textcolor{red}{This seems unfinished}
\begin{equation}
    \mathbf{T} = \begin{bmatrix} \mathbf{R} & \mathbf{t} \\ \mathbf{0}^\top & 1 \end{bmatrix}, \quad \mathbf{R} \in SO(3), \quad \mathbf{t} \in \mathbb{R}^3
\end{equation}


\subsubsection{EKF State Definition} The system state vector is:
\begin{equation}
    \mathbf{x} = \begin{bmatrix} \mathbf{p} & \dot{\mathbf{p}} & \mathbf{q} & \boldsymbol{\omega} \end{bmatrix}^\top
\end{equation}
where:
- $\mathbf{p} \in \mathbb{R}^3$: position $(x, y, z)$
- $\dot{\mathbf{p}} \in \mathbb{R}^3$: linear velocity $(v_x, v_y, v_z)$
- $\mathbf{q} \in \mathbb{H}$: unit quaternion $(q_x, q_y, q_z, q_w)$ for orientation
- $\boldsymbol{\omega} \in \mathbb{R}^3$: angular velocity $(\omega_x, \omega_y, \omega_z)$


\subsubsection{EKF State Prediction:}
\begin{align}
    \mathbf{x}_k &= \mathbf{F} \mathbf{x}_{k-1} + \mathbf{w}_k, \quad \mathbf{w}_k \sim \mathcal{N} (0, \mathbf{Q}) \\
    \mathbf{P}_k &= \mathbf{F} \mathbf{P}_{k-1} \mathbf{F}^\top + \mathbf{Q}
\end{align}
where $\mathbf{F}$ is the state transition matrix and $\mathbf{Q}$ is the process noise covariance.

\subsubsection{EKF State Update}
\begin{align}
    \mathbf{x}_k &= \mathbf{F} \mathbf{x}_{k-1} + \mathbf{w}_k, \\
    \mathbf{z}_k &= \mathbf{H} \mathbf{x}_k + \mathbf{v}_k
\end{align}
where $\mathbf{x}_k$ is the state, $\mathbf{z}_k$ is the observation, $\mathbf{F}$ is the motion model, $\mathbf{H}$ is the observation model, and $\mathbf{w}_k, \mathbf{v}_k$ are noise terms.

\subsubsection{Pose Update using FoundationPose (regaining object back to view)}
\begin{equation}
    \mathbf{T}_{\text{est}} = \operatorname{FoundationPose}(\text{image}, \mathbf{T}_{\text{EKF(t-1)}})
\end{equation}

\subsubsection{Optimal Viewpoint Sampling for Speedy Recovery}
\begin{equation}
    \mathbf{T}_{\text{sampled}} = \arg\max_{\mathbf{T}} \mathbb{E}[\operatorname{visibility}(\mathbf{T})]
\end{equation}

% \subsection{Pseudocode for Active Pose Estimation and Object Pose Recovery}

\begin{algorithm}
    \caption{Active Pose Estimation and Object Grasping}
\footnotesize
\begin{algorithmic}[1]
\State \textbf{Initialization:}
\State $t \gets 0$
\State $\mathcal{I}_t, \mathcal{D}_t$ : RGB, Depth images at time $t$
% \State $\mathcal{D}_t$ : Depth image at time $t$
\State $\mathcal{C}_t$ : Camera pose at time $t$
\State $\mathcal{G}_t^W, \mathcal{G}_t^C$ : Gripper pose in world \& camera frames at time $t$
\State $\mathcal{O}_\text{pool}^W, \mathcal{O}_\text{pool}^C$ : Grasp pose pool in world \& camera frames at time $t$
\State $\mathcal{O}_t^C$ : Grasp pose in camera frame at time $t$

\State $\mathcal{T}_t^W, \mathcal{T}_t^C$ : Object pose in world \& camera frames at time $t$
\State Read initial RGB-D image: $(\mathcal{I}_0, \mathcal{D}_0)$
\State Read text prompt $\mathcal{P}$ (e.g., “coffee cup”)
\State $\mathcal{B}_0 \gets \operatorname{GroundingDINO}(\mathcal{I}_0, \mathcal{D}_0, \mathcal{P})$
\State $\mathcal{M}_0 \gets \operatorname{2DTracker_{init}}(\mathcal{I}_0, \mathcal{B}_0)$
\State $\mathcal{T}_0^{C} \gets \operatorname{FoundationPose}(\mathcal{I}_0, \mathcal{D}_0, \mathcal{M}_0)$
\State $\mathcal{O}_\text{pool}^{W} \gets \operatorname{ContactGraspNet}(\mathcal{I}_0, \mathcal{D}_0)$
\State $\mathcal{O}_\text{pool}^{C} \gets \operatorname{TransformToCameraFrame}(\mathcal{C}_0, \mathcal{O}_\text{pool}^{W})$
\State $\mathcal{O}_{0}^{C} \gets \operatorname{SelectBestGrasp}(\mathcal{G}_0^C, \mathcal{O}_\text{pool}^C)$
\State $\mathcal{T}_\text{obj\_grasp}^C \gets \operatorname{ComputeTransform}(\mathcal{T}_0^C, \mathcal{O}_0^C)$
\State Initialize EKF with state $\mathbf{x}_0$, covariance matrix $\mathbf{P}_0$
\State $\text{use\_foundationpose} \gets \textbf{False}$
\State $\text{handover} \gets \textbf{False}$

\While {$\text{handover} = \textbf{False}$ and $t < t_{\max}$}
    \State $t \gets t+1$
    \State Read new RGB-D frame: $(\mathcal{I}_t, \mathcal{D}_t)$
    \State $\mathcal{M}_t, \mathcal{B}_t \gets \operatorname{2DTracker_{track}}(\mathcal{I}_t)$

    \If {$\mathcal{M}_t \neq \textbf{None}$}  
        \If {$\text{use\_foundationpose} = \textbf{True}$}  
            \State $\mathcal{T}_t^C \gets \operatorname{FoundationPose}(\mathcal{I}_t, \mathcal{D}_t, \mathcal{M}_t, \mathcal{T}_{t-1}^C)$
        \Else  
            \State $\mathcal{T}_t^C \gets \operatorname{BundleTrack\_R2D2}(\mathcal{I}_t, \mathcal{D}_t, \mathcal{M}_t, \mathcal{T}_{t-1}^C)$
        \EndIf
        \State $\mathcal{T}_t^W \gets \operatorname{}(\mathcal{C}_t *\mathcal{T}_t^C)$
        \State $\operatorname{EKF.update}(\mathcal{T}_t^W)$
    \Else  
        \State $\text{use\_foundationpose} \gets \textbf{True}$
        \State $\mathcal{T}_t^W \gets \operatorname{EKF.predict}()$
        \State $\mathcal{T}_t^C \gets \operatorname{}(inverse(\mathcal{C}_t) * \mathcal{T}_t^W)$
    \EndIf  

    \State $\mathcal{O}_t^C \gets \mathcal{T}_\text{obj\_grasp}^C \cdot \mathcal{T}_t^C$
    \State $\mathcal{O}_t^C \gets \operatorname{SelectBestGrasp}(\mathcal{G}_t^C, \mathcal{O}_t^C)$
    \State Move robot gripper toward $\mathcal{O}_t^C$

    \If {$\operatorname{Align}(\mathcal{G}_t^C, \mathcal{O}_t^C) = \textbf{True}$ and $\operatorname{Dist}(\mathcal{G}_t^C, \mathcal{O}_t^C) < \epsilon$}
        \State Grasp the object and lift
        \If {Grasping Failed} 
            \State Invoke RL Policy and continue
        \Else
            \State Grasping Success!!
            \State $\text{handover} \gets \textbf{True}$
        \EndIf
    \EndIf  
\EndWhile
\end{algorithmic}

\end{algorithm}

% \begin{algorithm}
% \caption{Active Pose Estimation and Recovery}
% \small
% \begin{algorithmic}[1]
% \State \textbf{Initialization:}
% \State $t\leftarrow 0$
% \State $I_t \text{: RGB Image at time } t$
% \State $D_t \text{: Depth Image at time } t$
% \State $C_t \text{: Camera Pose at time } t$
% \State $E^W_t \text{: Gripper Pose in World Frame at time } t$
% \State $E^C_t \text{: Gripper Pose in Camera Frame at time } t$
% \State $G^C_t \text{: Object Grasp Pose in Camera Frame at time } t$
% \State $GP^W_t \text{: Object Grasp Pose Pool in World Frame at time } t$
% \State $GP^C_t \text{: Object Grasp Pose Pool in Camera Frame at time } t$
% \State $T^W_t \text{: Object Pose in World Frame at time } t$
% \State $T^C_t \text{: Object Pose in Camera Frame at time } t$
% \State Read $(I_0, D_0)$ from the camera
% \State Read a text prompt $P$ (e.g., ``coffee cup")
% \State $BBox_0 \gets \operatorname{GroundingDINO}(I_0, D_0, P)$
% \State $Mask_0 \gets \operatorname{2DTracker_{init}}(I_0, BBox_0)$
% \State $T_0 \gets \operatorname{FoundationPose}(I_0, D_0, M_0)$
% \State $GP_{0}^{W} \gets \operatorname{ContactGraspNet}(I_0, D_0)$
% \State $GP_{0}^{C} \gets Inverse(C_{0})*GP_{0}^{W}$
% \State $G_{0}^{C} \gets \operatorname{Identify Best Grasp}(E_{0}^{C}, GP_0^{C})$
% \State $Tr_{OG}^C \gets \text{Object Pose to Grasp Pose Transform in Camera Frame}$
% \State Initialize the EKF with state $\mathbf{x}_0$, covariance matrix $\mathbf{P}_0$
% \State $\operatorname{use\_foundationpose} \gets False$
% \State $handover \gets False$


% \While {handover is False and $t< t_{max}$}
%     \State $t\leftarrow t+1$
%     \State Read $(I_t, D_t)$ from the camera 
%     \State $M_t, BBox_t \gets \operatorname{2DTracker_{track}(I_t)}$
%     \If {$M_t$ is not None}
%         \If {use\_foundationpose is True}
%             \State $\text{\# Mask is available as object came back to view}$
%             \State $T_t^{C} \gets \operatorname{FoundationPose}(I_t, D_t, M_{t}, T_{t-1}^C)$
%         \Else 
%             \State $T_t^{C} \gets \operatorname{BundleTrack\_R2D2}(I_t, D_t, M_t, T_{t-1}^C)$

%         \EndIf
%             \State $T_{t}^{W} \gets C_t * T_{t}^C$
%             \State $\operatorname{EKF.update}(T_{t}^{W})$
%     \Else
%         \State $use\_foundationpose \gets True$
%         \State $T_{t} \gets \operatorname{EKF.predict}()$
%         \State $T_{t}^{C} \gets \operatorname{inverse}(C_t) * T_t^W$
%     \EndIf
%     \State $GP_{t}^{C} \gets Tr_{OG}^C * T_t^C$
%     \State $G_{t}^{C} \gets \operatorname{IdentifyBestGrasp}(E_t^C, GP_t^C)$
%     \State Move the robot's Gripper toward $G_t^C$
%     \If {$\operatorname{align}(E_t^{C}, G_t^{C}) \text{ is True and dist}(E_t^{C}, G_t^{C}) < \epsilon$}
%         \State Grasp the Object and Lift it
%         \State $handover \gets True$
%     \EndIf
% \EndWhile
% \end{algorithmic}
% \end{algorithm}




% In the original system, pose of the target object is initialized in two steps: 1) User needs to manually draw a bounding box to generate the object mask. 2) User needs to manually provide a few points on the object's point cloud which serves as an initial pose estimate for BundleTrack to register the pose of the target object. We have removed the need to do those steps manually. For the first step, to perform zero-shot open-vocabulary object segmentation, we are using Grounding DINO~\cite{gdino} to automatically generate bounding box and use that information to produce a refined mask using SAM-HQ~\cite{sam-hq}. For the second step, we are using FoundationPose to give us an initial pose estimate of the target object. By reducing the number of Pose Hypothesis to less than 60, we can send quick and accurate enough initial estimate of the pose for Bundle Track and R2D2 to start tracking the object pose and mask respectively. FoundationPose performs offline/video pose estimation and tracking. Hence, We have modified it to work for an online setting, where image data is actively streamed and 6D pose is estimated on demand. Moreoften that not, the tracker in FoundationPose is unstable as in our setup, both the camera and target object randomly move in 3D space and we believe our setup produces target object trajectories that FoundationPose's pose refiner model would not have seen during in its training data.

% In the original system, initializing the target object's pose required two manual steps: (1) drawing a bounding box to generate the object mask, and (2) selecting key points on the object's point cloud to provide an initial pose estimate for BundleTrack. We automate both steps to streamline the process. 
%Initially, for the first image frame (RGB-D), we employ Grounding DINO~\cite{gdino} to automatically generate a bounding box by prompting it with the name of the target object. We then send the RGB and the bounding box to a 2D Object Tracker to produce and track the mask of the target object. 
% , refining the mask with SAM-HQ~\cite{sam-hq}. 
%We leverage FoundationPose, which provides an initial pose estimate of the target object. 

\subsubsection{Object tracking during out-of-view}
% When the object goes out of view, we lose the mask of the object and hence pose tracking fails and pose produced by Bundle Track would no longer be accurate and hence, the EARL policy will not be able to successfully grasp and often results in collision with the wall or self-collision of the robot arm. To address this, we leveraged a non-linear model to estimate the 6D pose of the target based on the pose data we have so far. Specifically, we are using Extended Kalman Filter (EKF) assuming constant 3D velocity for the target object. Pertaining to the workspace limitations, we have deduced a good step size for the Kalman pose update. The policy does not know if the object went out of view, as we provide the pose generated by the Kalman Filter as the target object pose for it reach and grasp. We have 
When the object moves out of view, we lose its mask, causing BundleTrack to produce inaccurate pose estimates. As a result, the policy will fail to grasp the object, often leading to collisions with the nearby wall or self-collisions of the robot arm. To address this, we employ a non-linear model—specifically, an Extended Kalman Filter (EKF) assuming a constant 3D velocity for the target object, to estimate its 6D pose based on pose data tracked/recorded so far. Given workspace constraints for the boundaries of the target object, we are required determine an optimal step size for Kalman updates. KARL policy remains unaware that the object has gone out of view, as it continues receiving pose estimates from the Kalman Filter. However, two key challenges arise: 

\begin{itemize}
\item \textbf{Guiding the robot towards regaining visual contact:}  The predicted pose trajectory must direct the robot correctly to regain sight of the target. As long as the measurements fed into the Kalman Filter contain approximately constant 3D velocities of the object, the predicted estimates point can guide the policy in the right direction. Since, the policy performs a top-down grasping, correct direction is not sufficient as target object might be bordering next to the horizontal FoV of the camera. Hence, instead of relying solely on the mean of the EKF's estimated pose distribution, we sample a pose that maximizes the expected view of the uncertain region, thereby enhancing the likelihood of recovering the lost target.
\item \textbf{Maintaining Update Balance:} The Kalman Updates should not be huge as large pose changes will trick the policy and cause unwanted behaviors. The largest velocity change between two frames seen during policy training is less than 3cm/s, more than which usually easily gets object out of view (as the robot is closely following the target object). At the same time, Kalman Updates cannot be small as the policy might prematurely execute a swift grasp at a false pose as it thinks object is appearing to move slowly. We tackle this by selecting an optimal step size that strikes the necessary balance.
\end{itemize}
By balancing these factors, our approach significantly improves target reacquisition while reducing erratic policy behaviors and premature grasp attempts at positions where the object is absent.


\subsubsection{Object Tracking Recovery}
Once the Extended Kalman Filter (EKF) successfully guides the robot to regain visual contact with the object, we leverage R2D2 to confirm the object's mask availability. Instead of re-registering the pose with BundleTrack—which is computationally expensive—we use FoundationPose for efficient and accurate pose estimation. To streamline recovery, we assume the object remains stationary or undergoes minimal motion once it leaves the field of view. This prevents unnecessary re-tracking. If slight movement occurs, we repeatedly invoke FoundationPose's pose estimator to update the object's pose. Since FoundationPose's tracker is unreliable for our setup, we further accelerate its estimation by reusing the last known XYZ position with a reduced set of hypotheses. This enables fast, iterative pose estimation, ensuring the robot successfully grasps the target without delays.

% Upon successful pose guidance from the Extended Kalman Filter, when objects gets visible in the view of the camera (We rely on R2D2 tracker to signal the availability of the object mask), instead of registering pose using BundleTrack (which is costly/time consuming), we use FoundationPose to accurately register the new pose of the target object. Once the object goes out of view, we are assuming the object stays still with no or minimal pose changes. This avoids tracking the object again. In case, the object moves slightly, we repetitively call FoundationPose's pose estimator to track the pose. Since, the pose tracker from FoundationPose cannot reliably track for our setup, we make FoundationPose's pose estimation even faster by reusing the last saved pose's XYZ information as the XYZ again using a smaller number of hypothesis and perform quick repetitive pose estimation until successful grasp of the target by the robot. 

==> texs/04-backup.tex <==
To comprehensively evaluate the performance of our proposed method, we designed six sets of experiments—five in simulation and one in a real-world setting. These experiments introduce different levels of complexity through: 
{\bf Experiment A}: We study the impact of target object speeds, by gradually increasing it.
{\bf Experiment B}: We study the impact of stricter grasping time constraints.
{\bf Experiment C}: We expanded the target object workspace.
{\bf Experiment D}: Target object tracking loss conditions are challenged. 
{\bf Experiment E}: An ablation study assessing the impact of the previous four factors when combined.
{\bf Experiment F}: Real-world evaluation using a physical robot.


\textbf{Target Object Motion:} 
The target object is initially placed at one boundary of the workspace with a sampled 6D pose and follows one of two motion patterns:
\begin{itemize}
    \item \textbf{Linear Motion (Regular):} The object moves at a constant speed between 0 cm/s and 5 cm/s with no rotational motion. $70\%$ of the trials in \textbf{Experiments B and C} consider moving objects in this motion.
    \item \textbf{Linear Motion (Fast):} The object moves at a higher constant speed, up to 15 cm/s, maintaining zero rotational velocity.
    \item \textbf{Random Motion:} The object moves with a maximum translational velocity of 5 cm/s while undergoing random rotations between 0° and ~14.5° in clockwise or anticlockwise direction along the X, Y, and Z axes. In the simulation, the object never fully halts; even when its velocity decreases at random intervals, it continues to exhibit slight oscillations around its center of mass, introducing an element of unpredictability. $30\%$ of the trials in \textbf{Experiments B and C} consider moving objects in this motion.
    \item \textbf{Disruptive Motion:} To simulate tracking loss scenarios, the object's velocity abruptly increases to 30 cm/s or higher, causing it to move out of the camera's field of view before coming to a complete stop. 
\end{itemize}

\subsection{Higher Object Speeds}
We evaluated KARL’s grasping performance under increasing linear motion speeds (3 cm/s to 15 cm/s). KARL maintained a near-perfect success rate ($>$99\%) with zero collisions for speeds up to 9 cm/s. We attribute this to its emphasis on rewarding successful grasp closures. At higher speeds, KARL still outperformed EARL, achieving a 92.58\% success rate when the object's speed was sampled uniformly between 0–15 cm/s. While EARL struggled with tracking failures at higher speeds, KARL's EKF module prevented these issues, ensuring robust object tracking and grasp execution. (See Table~\ref{tab:obj_speed}).

 
\setlength{\tabcolsep}{4.1pt}
\begin{table}[htbp]
\caption{Performance comparison of EARL and KARL under different target object speeds over 1000 Isaac Gym Simulation Environments}
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{llccccccc}
\toprule
\multirow{2}{*}{\;} & \multirow{2}{*}{Policy} & \multicolumn{6}{c}{Target Object Speed (cm/s)} \\ 
\cmidrule(lr){3-8} 
                        &                         & 3  & 6  & 9  & 12  & 15   & Random \\ 
\midrule
\multirow{2}{*}{Success ($\uparrow$)} & EARL                     & 94.38   & 95.40   &  95.83  &  80.22  &  64.64  &  89.21  \\  
                         & KARL              & \textbf{99.21}   & \textbf{99.33}   &  \textbf{99.10}  & \textbf{82.81}   & \textbf{67.34}   & \textbf{92.58}   \\ 
\midrule
Time Limit  & EARL                 & \textbf{0.45}   &  1.35  & \textbf{1.13}   & \textbf{1.01}   & \textbf{0.68}   & \textbf{0.79}   \\  
(35 sec) ($\downarrow$)                                     & KARL       & 0.79   &  \textbf{0.67}  & 0.90   &  8.65  & 14.08   &  3.82  \\  
\midrule
\multirow{2}{*}{Collision ($\downarrow$)} & EARL                   &  0.11  & 0.22  & 0.11   & \textbf{3.93}   & \textbf{5.63}   & \textbf{1.12}   \\  
                           & KARL         & \textbf{0.0}   &  \textbf{0.0}  & \textbf{0.0}   & 8.54   &  18.58  & 3.60   \\  
\midrule
Tracking  & EARL            &  5.06  & 3.03   & 2.93   & 14.83   &  29.05  &  8.88  \\  
Failure ($\downarrow$)          & KARL     & \textbf{0.0}   & \textbf{0.0}   & \textbf{0.0}   & \textbf{0.0}   & \textbf{0.0}   & \textbf{0.0}   \\  
\midrule
Total & EARL              &  5.62  & 4.60   & 4.17   & 19.78   & 35.36   &  10.79  \\  
Failure ($\downarrow$)                               & KARL       & \textbf{0.79}   &  \textbf{0.67}  & \textbf{0.90}   & \textbf{17.19}   & \textbf{32.66}   &  \textbf{7.42}  \\  
\bottomrule
\end{tabular}
\label{tab:obj_speed}
\end{table}

% We have considered constant velocity linear motions of increasing speed (3cm/s to 12cm/s) and observed that KARL demonstrated improved grasping success rate with over $99\%$ success rate and $0\%$ collision rate for speeds up to $9cm/s$. We attribute this to considering higher reward for successfully closing the gripper.   Settting aside these individual categories, we also chose a category setting the target object speed uniformly randomly from $0cm/s$ to $12cm/s$, and observed that KARL achieves over $92\%$ success rate.
% \begin{table}[htbp]
% \caption{\textcolor{red}{I will update this after finishing all the todos}
% Performance comparison of EARL and KARL under different target object speeds over 1000 Isaac Gym Simulation Environments}
% \label{tab:obj_speed}
% \centering
% \scalebox{0.85}{
% \renewcommand{\arraystretch}{1.2}
% \begin{tabular}{llccccc}
% \toprule
% \multirow{2}{*}{Metric (\%)} & \multirow{2}{*}{Policy} & \multicolumn{5}{c}{Target Object Speed (cm/s)} \\ 
% \cmidrule(lr){3-7} 
%                         &                         & 3  & 6  & 9  & 12  & 0-15 \\ 
% \midrule
% \multirow{2}{*}{Success ($\uparrow$)} & EARL                     & 94.38   & 95.40   &  95.83  &  80.22  &  89.21  \\  
%                          & KARL (Ours)              & \textbf{99.21}   & \textbf{99.33}   &  \textbf{99.10}  & \textbf{82.81}   & \textbf{92.58}   \\ 
% \midrule
% \multirow{2}{*}{Time Limit (35 sec) ($\downarrow$)} & EARL                 & \textbf{0.45}   &  1.35  & \textbf{1.13}   & \textbf{1.01}   & \textbf{0.79}   \\  
%                                      & KARL (Ours)         & 0.79   &  \textbf{0.67}  & 0.90   &  8.65  &  3.82  \\  
% \midrule
% \multirow{2}{*}{Collision ($\downarrow$)} & EARL                   &  0.11  & 0.22  & 0.11   & \textbf{3.93}   & \textbf{1.12}   \\  
%                            & KARL (Ours)           & \textbf{0.0}   &  \textbf{0.0}  & \textbf{0.0}   & 8.54   & 3.60   \\  
% \midrule
% \multirow{2}{*}{Tracking Failure ($\downarrow$)} & EARL            &  5.06  & 3.03   & 2.93   & 14.83   &  8.88  \\  
%                                   & KARL (Ours)    & \textbf{0.0}   & \textbf{0.0}   & \textbf{0.0}   & \textbf{0.0}   & \textbf{0.0}   \\  
% \midrule
% \multirow{2}{*}{Total Failure ($\downarrow$)} & EARL              &  5.62  & 4.60   & 4.17   & 19.78   &  10.79  \\  
%                                & KARL (Ours)      & \textbf{0.79}   &  \textbf{0.67}  & \textbf{0.90}   & \textbf{17.19}   &  \textbf{7.42}  \\  
% \bottomrule
% \end{tabular}
% }
% \end{table}


\begin{table}[htbp]
\caption{Performance comparison of EARL and KARL under different time limits over 1000 Isaac Gym Simulation Environments}
\centering
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{lcc}
\toprule
\textbf{\;} & \textbf{EARL (\%)} & \textbf{KARL (Ours) (\%)} \\  
\midrule
Success ($t \leq 35s$) ($\uparrow$) & 95.16 & \textbf{96.89} \\
Success ($t \leq 30s$) ($\uparrow$) & 93.61 & \textbf{96.34} \\
Success ($t \leq 25s$) ($\uparrow$) & 93.54 & \textbf{96.17} \\
Success ($t \leq 20s$) ($\uparrow$) & 91.91 & \textbf{94.14} \\
Success ($t \leq 15s$) ($\uparrow$) & 84.46 & \textbf{91.83} \\
Success ($t \leq 10s$) ($\uparrow$) & 21.03 & \textbf{26.70} \\
Success ($t \leq 5s$) ($\uparrow$) & \textbf{0} & \textbf{0} \\
\midrule
Timeout ($>35s$) ($\downarrow$) & 2.70 & \textbf{2.32} \\
Collision ($\downarrow$) & \textbf{0.79} & \textbf{0.79} \\
Tracking Failure ($\downarrow$) & 1.35 & \textbf{0.0} \\
Total Failure ($\downarrow$) & 4.84 & \textbf{3.11} \\
\bottomrule
\end{tabular}
\label{tab:time_limit}
\end{table}
\subsection{Decreased Task Time limits}
We evaluated KARL’s grasping success under progressively tighter time constraints, ranging from 35 to 5 seconds (refer to TABLE~\ref{tab:time_limit}). In $70\%$ of the trials, objects followed regular linear motions and followed random trajectories in the remaining trials. KARL achieves a $91.83\%$ success rate within 15 seconds, outperforming EARL, which reaches similar performance at 20 seconds—a 5-second advantage. Notably, $99.9\%$ of KARL’s successful grasps occurred within 25 seconds, consistently outperforming EARL across all time limits. Interestingly, neither KARL nor EARL succeeded in completing the grasping task within 5 seconds. However, beyond this extreme constraint, KARL also exhibited zero tracking failures and a lower overall failure rate, demonstrating significant robustness in time-constrained grasping scenarios.



\setlength{\tabcolsep}{5.7pt}
\begin{table}[htbp]
\caption{Performance comparison of EARL and KARL on the Enlarged KARL's Workspace ($W_{KARL} = W_{EARL} + W_A + W_B$) over 1000 Isaac Gym Simulation Environments}
\centering
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{llcccccc}
\toprule
\multirow{2}{*}{Metric (\%)} & \multirow{2}{*}{Policy} & \multicolumn{5}{c}{Target Object Workspace} \\ 
\cmidrule(lr){3-7} 
                        &                         & $W_A$  & $W_B$  & $W_{EARL}$  &  $W_{KARL}$ \\ 
\midrule
\multirow{2}{*}{Success ($\uparrow$)} & EARL                   &  78.01  & 84.24   & 95.09   & 81.67   \\  
                         & KARL                 &  \textbf{97.16}  &  \textbf{97.41}   & \textbf{96.89}   & \textbf{90.47}   \\  
\midrule
Timeout & EARL          & 11.45   & 3.28  &  2.77  & 12.04     \\  
(35 sec) ($\downarrow$)                                     & KARL      & \textbf{2.03}   &  \textbf{1.85}  & \textbf{2.32}   & \textbf{7.10}   \\  
\midrule
\multirow{2}{*}{Collision ($\downarrow$)} & EARL                  & 1.53   &  1.67  & \textbf{0.79}   & \textbf{2.27} &   \\  
                           & KARL              &  \textbf{0.81}  &  \textbf{0.74}  & \textbf{0.79}   & 2.43   \\  
\midrule
Tracking  & EARL           & 9.01   & 10.81   & 1.35   & 4.02  \\  
Failure ($\downarrow$)                                  & KARL          & \textbf{0.0}    &  \textbf{0.0}   &  \textbf{0.0}   & \textbf{0.0}   \\  
\midrule
Total  & EARL              &  21.99  &  15.76  & 4.91  & 18.33   \\  
Failure ($\downarrow$)                               & KARL             &  \textbf{2.84}  &  \textbf{2.59}  & \textbf{3.11}  & \textbf{9.53}   \\  
\bottomrule
\end{tabular}
\label{tab:workspace}
\end{table}

\subsection{Enlarged Workspace}
% We expanded EARL's workspace and doubled the operational volume by adding two new partitions. 
We expanded EARL's target object workspace $W_{EARL}$ by considering two adjacent workspaces $W_A$ and $W_B$.
% partitions—A (40 × 20 × 40 $cm^3$) and B (40 × 10 × 40 $cm^3$)—

nearly doubling the operational volume and we call it KARL's workspace. 
% In 70\% of the trials, objects followed regular linear motions and followed random trajectories in the rest of trials. 
Both KARL and EARL are trained on EARL's workspace for fair comparison. As seen in Table \ref{tab:workspace}, EARL struggled significantly in the new partitions, with failures primarily due to timeouts and tracking losses. In contrast, KARL maintained a grasping success rate of $~97\%$ across all partitions, showing superior adaptability. In KARL's workspace, where the effective range is increased from 40 cm to 70 cm, KARL experienced increased timeouts but still outperformed EARL across all metrics. KARL had zero tracking failures and consistently lower collision rates, proving its adaptability in larger, more challenging workspaces.

\setlength{\tabcolsep}{4.8pt}
\begin{table}[htbp]
\caption{Performance comparison of EARL and KARL on regular and tracking loss scenarios over 1500 Isaac Gym Simulation Environments}
\centering
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{llcccccc}
\toprule
\multirow{2}{*}{Metric (\%)} & \multirow{2}{*}{Policy} & \multicolumn{5}{c}{Scenarios (\#)} \\ 
\cmidrule(lr){3-7} 
                        &                         & \makecell{Line \\ (700)}  & \makecell{Random \\ (300)}  & \makecell{Tracking \\ Loss (500)}  & \makecell{Overall \\ (1500)} \\ 
\midrule
\multirow{2}{*}{Success ($\uparrow$)} & EARL                   &  94.60  & 96.0   & 7.10   & 65.72   \\  
                         & KARL                  &  \textbf{96.10}  &  \textbf{98.50}   & \textbf{94.30}   & \textbf{95.98}   \\  
\midrule
Timeout & EARL          & 3.70   & 0.6  &  \textbf{0.0}  & \textbf{1.85}     \\  
(35 sec) ($\downarrow$)                                     & KARL     & \textbf{3.10}   &  \textbf{0.5}  & 5.20   & 3.28   \\  
\midrule
\multirow{2}{*}{Collision ($\downarrow$)} & EARL                  & 1.5   &  2.4  & 1.8   & 1.17 &   \\  
                           & KARL              &  \textbf{0.8}  &  \textbf{1.0}  & \textbf{0.5}   & \textbf{0.74}   \\  
\midrule
Tracking & EARL           & 1.5   & 1.0   & 91.10   & 31.27  \\  
Failure ($\downarrow$)                                  & KARL          & \textbf{0.0}    &  \textbf{0.0}   &  \textbf{0.0}   & \textbf{0.0}   \\  
\midrule
\multirow{2}{*}{Total Failure ($\downarrow$)} & EARL              &  5.40  &  4.0  & 92.90  & 34.29   \\  
                               & KARL            &  \textbf{3.9}  &  \textbf{1.5}  & \textbf{5.7}  & \textbf{4.02}   \\  
\bottomrule
\end{tabular}
\label{tab:tracking_loss}
\end{table}

\subsection{Tracking Loss}
Beyond the workspace expansion and the tighter time constraints, we further assessed KARL’s resilience to objects exiting the camera’s view—one of the unavoidable circumstances in dynamic grasping. We ran 1,500 simulations: 1,000 with regular object motion and 500 where objects suddenly accelerated beyond 20 cm/s, forcing them out of view to simulate extreme tracking loss. Once out of view, objects remained stationary until the experiment ended. In the regular motion trials (700 with constant speeds of 0–5 cm/s and 300 with random trajectories), objects could exit the view, but only incidentally. 
TABLE~\ref{tab:tracking_loss} shows that while EARL performs well under regular motion (94.6\% success), its success rate plummets to 7.1\% in tracking loss scenarios, failing to recover lost object poses. In contrast, KARL, equipped with EKF, accurately extrapolates the object's motion, leading to an impressive 94.3\% success rate even under tracking disruptions. The robot follows the predicted path produced by the EKF and reaches the target. However, EKF's update size cannot be tuned for different object speeds and the robot might reach the end of the episode before reaching the object. This can be observed in KARL's timeout rate. KARL exhibits zero tracking failures and consistently outperforms EARL across all scenarios.

% In this experiment, we conducted 1,500 simulation tests, where 1000 trails involve regular object motion. With the overall object motion trajectory staying linear, in the remaining 500 trials, objects were suddenly accelerated beyond 20 cm/s, moving out of view—simulating extreme tracking loss. Once the object is out of view, it halts until the end of the experiment. In the regular motion (700 of which feature constant-speed object motion (0-5 cm / s) and 500 of which follow random trajectories), object can still go out of view, however it can only happen by accident. 
% In this experiment, we have consider 1500 simulation trials of which, in 700 of them, objects were moved at constant speeds (0–5 cm/s) and in 500 of them objects moved in random trajectories, however in the rest of 500 trails, object certainly goes out of view by suddenly moving at 20 cm/s or more to jump out of sight of the camera and halts there until the end of the trail, the overall trajectory is still linear. Although behind KARL, while EARL shows good performance on regular object motions (over 94\% success rate), its performance drops to mere $7.10$ and cannot recover the object back into the view of the camera. KARL, with EKF in place, accurately extrapolates this linear path incrementally leading to the accurate jumped goal position. KARL shows minimal drop in performance on the tracking loss scenarios with over $94\%$ success rate and primary reason for failure is timeout and this attributed to the kalman update size on the predicted pose. However, EKF is still optimized to ensure high success rate overall.  

\setlength{\tabcolsep}{3pt}
\begin{table}[]
\caption{Ablation study on the new scene setup (larger workspace, higher object speeds, tracking loss scenarios) over 1000 Isaac Gym Simulation Environments}
\label{tab:ablation}
\centering
\begin{tabular}{lccccc}
\toprule
\multirow{2}{*}{Policy} & \multicolumn{5}{c}{Metric (\%)}                                  \\
                        & Success ($\uparrow$) & Timeout($\downarrow$)& Collision($\downarrow$)& 
                        \makecell{Tracking \\Failure($\downarrow$)}& \makecell{Total\\Failure($\downarrow$)}\\
\midrule
EARL                    & 66.29   & 7.84    & 2.54      & 23.32            & 33.71         \\
Old Cur. & 76.70   & 15.21   & 8.08      & \textbf{0.00}       & 23.30         \\
No EKF            & 72.62   & \textbf{4.00}    & \textbf{2.27}      & 21.11            & 27.38         \\
KARL                     & \textbf{83.46}   & 10.46   & 6.08      & \textbf{0.00}       & \textbf{16.54}         \\
\bottomrule
\end{tabular}
\end{table}

\subsection{Ablation Study on KARL}
After independently evaluating KARL across various challenging scenarios, we now assess its performance when all three difficulties—expanded workspace, increased object speeds, and tracking loss scenarios—are combined, making the task significantly more demanding. 

In this setup, the objects primarily move within the enlarged workspace. 70\% of the time, the object moves at constant speeds between 0 cm/s and 15 cm/s and is forced out of view with a 30\% probability. We did not choose to further increase the out-of-view probability in order to keep the simulation realistic.   
% Initially, it moves at constant speeds between 0 cm/s and 15 cm/s, but at random intervals, its speed increases to 30 cm/s, intentionally causing tracking loss.
For the remaining 30\% of trials, the object follows a random trajectory, where it may exit the camera's view inadvertently.

To further analyze KARL’s performance, we conducted an ablation study by systematically removing key components—EKF (for tracking loss recovery) and the new curriculum (for better grasp adaptation)—to isolate their contributions.

As shown in Table \ref{tab:ablation},
KARL without the new curriculum (but with EKF) eliminates tracking failures and improves upon EARL by a 10\% higher success rate, but timeouts remain a challenge. This is partially due to EKF update size limitations and partially due to the lack of imprecise gripper alignment avoidance in EARL with the object's grasp pose.
    KARL without EKF (but with the new curriculum) reduces gripper misalignment issues, decreasing timeouts and improving the success rate by 6\% over EARL. However, without EKF, tracking failures remain high, only slightly lower than EARL.
    KARL achieves the highest success rate (83.46\%), improving upon EARL by 17.17\%, with zero tracking failures and a significantly lower overall failure rate.

These results reinforce the importance of both EKF for robust object tracking recovery and the new curriculum for improved grasp alignment and success, demonstrating that their combined effect enables KARL to outperform EARL across all difficulty levels.



\begin{table}[htbp]
\caption{Real-world comparison of EARL and KARL}
\label{tab:real_exp}
\centering
\begin{tabular}{lllll}
\toprule
\multirow{2}{*}{Policy} & \multicolumn{2}{c}{Success} & \multicolumn{2}{c}{Premature Grasping} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5}
                        & Regular                   & Complex                  & Regular            & Complex            \\
\midrule
EARL                    & 60                       & 53.3                     & -                 & -                  \\
% EARL + Pose Switch      & 60                       & 53.3                     & -                 & -                  \\
\textbf{KARL}           & \textbf{93.3}            & \textbf{80}              & \textbf{0}        & \textbf{6.6}       \\
% \textbf{KARL + Pose Switch} & \textbf{93.3}       & \textbf{80}              & \textbf{0}        & \textbf{6.6}       \\
\bottomrule
\end{tabular}
\end{table}

\subsection{Real Robot Experiments}
To validate KARL’s real-world performance, we conducted grasping experiments using a UR5e robotic arm equipped with a 2F-85 Robotiq Gripper. Each policy—KARL and EARL—was tested in 30 trials, totaling 60 trials across different scenarios.
These trials included:
\begin{itemize}
    \item \textbf{Regular Scenes (15 trials):} The only object in the scene was the target object, with no obstacles.
    \item \textbf{Complex Scenes (15 trials):} The target moved behind obstacles such as shelves or walls, requiring the robot to follow and maintain visibility, highlighting the advantage of an Eye-on-Hand (EoH) system. However, explicit collision avoidance was not in place, introducing the potential for unintended contact.
\end{itemize}
Additionally, the target object's motion followed one of three patterns:
\begin{itemize}
    \item 14 trials with linear motion,
    \item 6 trials with random motion,
    \item 10 trials where tracking was intentionally lost, forcing the robot to recover the object’s location.
\end{itemize}
As shown in Table \ref{tab:real_exp}, KARL outperforms EARL in both regular and complex scenarios. In obstacle-free conditions, KARL achieves an impressive 93.3\% success rate, while EARL struggles at 60\%. In complex environments, KARL maintains a strong 80\% success rate, whereas EARL drops to 53.3\%. EARL falters mainly due to its inability to recover objects that move out of view.

One observed limitation of KARL is premature grasping—in 6.6\% of complex scene trials, KARL attempted to grasp an estimated pose from its EKF-based predictions before reaching the actual object. Unlike in simulation, where successful grasping is confirmed through object contact, our real-world setup lacks this feature, leading to occasional early grasp attempts.

These results reinforce the findings from the simulation studies—KARL’s EKF-based tracking and adaptive grasping curriculum provide significant advantages, especially in dynamic and occlusion-heavy environments. While minor real-world limitations exist, KARL consistently outperforms EARL across all tested conditions, demonstrating superior robustness and adaptability in real-world grasping tasks.
% We have evaluated KARL's performance on real grasping experiments using an UR5e robot attached with a 2F-85 Robotiq Gripper. We have conducted a total of 60 trails, 30 each for EARL and KARL respectively. 14 trials follow linear object motion, 6 random and 10 in a way object tracking gets lost, totaling 30 trials. 15 of these trails comprise regular scenarios where the only object in the scene is the target object and there is no obstacle. In the remaining 15 trails, we involve making the robot follow the target where it is eventually placed on a shelf or on another large object or going behind a wall to show the merit of an EoH system however there is room for collision as we do not have explicit collision avoidance in place. Outperforming EARL, KARL achieves a success rate of $93.3\%$ in a regular collision-free scenario. In the complex scenario as well, KARL acheives 80\% success rate. EARL struggles to produce good success rates as it completely fails for the trails involving object going out of view. For complex scenario, we have observed a premature grasping rate of 6.6\% for KARL as the robot can prematurely grasp the fake/predicted pose from EKF before reaching the target object. While this is avoidable in simulation as object contact with the gripper is ensured for successful grasping, but cannot be realized in a real experiment. 


% \begin{table*}[htbp]
% \caption{Performance comparison of EARL and KARL under different time limits over 1000 Isaac Gym Simulation Environments}
% \centering
% \scalebox{0.75}{
% \renewcommand{\arraystretch}{1.2}
% \begin{tabular}{llccccccccccc}
% \toprule
% \multirow{2}{*}{Policy} & \multicolumn{7}{c}{Success under different time limits $t$ (\%) ($\uparrow$)} & \multirow{2}{*}{Timeout (\%) ($>$35 sec) ($\downarrow$)} & \multirow{2}{*}{Collision (\%)  ($\downarrow$)} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Tracking \\ Failure (\%)  ($\downarrow$)\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Total \\ Failure (\%)  ($\downarrow$)\end{tabular}} \\  
% \cmidrule(lr){2-8} 
%                         & $t \leq 5s$ & $t \leq 10s$ & $t \leq 15s$ & $t \leq 20s$ & $t \leq 25s$ & $t \leq 30s$ & $t \leq 35s$ &  &  & &   \\  
% \midrule
% EARL & \textbf{0} & 21.03 & 84.46 & 91.91 & 93.54 & 93.61 & 95.16 & 2.70 & \textbf{0.79} & 1.35 & 4.84 \\  
% KARL (Ours) & \textbf{0} & \textbf{26.70} & \textbf{91.83} & \textbf{94.14} & \textbf{96.17} & \textbf{96.34} & \textbf{96.89} & \textbf{2.32} & \textbf{0.79} & \textbf{0.0} & \textbf{3.11} \\  
% \bottomrule
% \end{tabular}
% }
% \label{tab:KARL_performance}
% \end{table*}

